Measurement of the top quark mass in the $t\bar{t}\to$ lepton+jets channel from $\sqrt{s}=8$ TeV ATLAS data and combination with previous results

The top quark mass is measured using a template method in the $t\bar{t}\to$ lepton+jets channel (lepton is $e$ or $\mu$) using ATLAS data recorded in 2012 at the LHC. The data were taken at a proton-proton centre-of-mass energy of $\sqrt{s}=8$ TeV and correspond to an integrated luminosity of 20.2 fb$^{-1}$. The $t\bar{t}\to$ lepton+jets channel is characterized by the presence of a charged lepton, a neutrino and four jets, two of which originate from bottom quarks ($b$). Exploiting a three-dimensional template technique, the top quark mass is determined together with a global jet energy scale factor and a relative $b$-to-light-jet energy scale factor. The mass of the top quark is measured to be $m_{top}= 172.08 \pm 0.39 (stat) \pm 0.82 (syst)$ GeV. A combination with previous ATLAS $m_{top}$ measurements gives $m_{top}= 172.69 \pm 0.25 (stat) \pm 0.41 (syst)$ GeV.

==> app_auxil.tex <==
 In the following shown are auxiliary figures that we would like to make
 available to speakers presenting the analysis.
%
%--------------------------------------------------------------------------
\begin{figure*}[tbph!]
\centering
\includegraphics[width=0.48\textwidth]{ChiQuaAll}
%
\caption{Compatibilities of the 15 pairs ($i, j$) of the six measurements.
  The compatibility is calculated from  the measured values \xX{i}, \xX{j},
  the uncertainties \sigmaX{i}, \sigmaX{j}\ and the correlations \rhoX{ij},
  using
  $\chiqij=\frac{(x_i-x_j)^2}{\sigma_i^2+\sigma_j^2-2\rhoX{ij}\sigma_i\sigma_j}$.
%
}
\end{figure*}
%--------------------------------------------------------------------------
%
%--------------------------------------------------------------------------
\begin{figure*}[h!]
\centering
\includegraphics[width=0.48\textwidth]{TopMassInp}
%
\caption{The inputs to the combination, with the combined value added to the
  figure.
%
}
\end{figure*}
%--------------------------------------------------------------------------
%
%--------------------------------------------------------------------------
\begin{figure*}[tbp!]
\centering
\subfigure[Central values \mtsig]{
  \includegraphics[width=0.48\textwidth]{Stability_N3_Val}}
\subfigure[Uncertainties \mtsig]{
  \includegraphics[width=0.48\textwidth]{Stability_N3_Unc}}
\hfill
\subfigure[Central values \mt]{
  \includegraphics[width=0.48\textwidth]{Stability_Val}}
\subfigure[Uncertainties \mt]{
  \includegraphics[width=0.48\textwidth]{Stability_Unc}}
%
\caption{The results for the combined values and their uncertainties in 500
  combinations.
%
 The results for \mtsig\ are in the upper row, those for \mt\ in the lower one.
%
 The mean value and the root mean square of each distribution is also reported.
%
 The arrows indicate the combined value and the uncertainty for the original
 result.
%
 For each combination, the sizes of the uncertainties as well as the
 correlations are newly evaluated.
%
 For this, random variations are performed of each systematic uncertainty within
 the corresponding statistical precision.
%
 Caused by the re-evaluation of the correlation, the resulting distributions
 are not Gaussian and are also not exactly centred around the combined value and
 the combined uncertainty. This non-Gaussian behaviour is much smaller for
 \mt\ than for $\sigma(\mt)$, which exhibits a longer tail to larger values.
%
}
\end{figure*}
%--------------------------------------------------------------------------
%

